ModMag: A Modular Magnetic Micro-Robotic Manipulation Device

Electromagnetic systems have been used extensively for the control magnetically actuated objects, such as in microrheology and microrobotics research. Therefore, optimizing the design of such systems is highly desired. Some of the features that are lacking in most current designs are compactness, portability, and versatility. Portability is especially relevant for biomedical applications in which in vivo or in vitro testing may be conducted in locations away from the laboratory microscope. This document describes the design, fabrication and implementation of a compact, low cost, versatile, and user friendly device (the ModMag) capable of controlling multiple electromagnetic setups, including a two-dimensional 4-coil traditional configuration, a 3-dimensional Helmholtz configuration, and a 3-dimensional magnetic tweezer configuration. All electronics and circuitry for powering the systems is contained in a compact 10"x6"x3" system which includes a 10" touchscreen. A graphical user interface provides additional ease of use. The system can also be controlled remotely, allowing for more flexibility and the ability to interface with other software running on the remote computer such as propriety camera software. Aside from the software and circuitry, we also describe the design of the electromagnetic coil setups and provide examples of the use of the ModMag in experiments.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


